LipSim: A Provably Robust Perceptual Similarity Metric

Recent years have seen growing interest in developing and applying perceptual similarity metrics. Research has shown the superiority of perceptual metrics over pixel-wise metrics in aligning with human perception and serving as a proxy for the human visual system. On the other hand, as perceptual metrics rely on neural networks, there is a growing concern regarding their resilience, given the established vulnerability of neural networks to adversarial attacks. It is indeed logical to infer that perceptual metrics may inherit both the strengths and shortcomings of neural networks. In this work, we demonstrate the vulnerability of state-of-the-art perceptual similarity metrics based on an ensemble of ViT-based feature extractors to adversarial attacks. We then propose a framework to train a robust perceptual similarity metric called LipSim (Lipschitz Similarity Metric) with provable guarantees. By leveraging 1-Lipschitz neural networks as the backbone, LipSim provides guarded areas around each data point and certificates for all perturbations within an $\ell_2$ ball. Finally, a comprehensive set of experiments shows the performance of LipSim in terms of natural and certified scores and on the image retrieval application. The code is available at https://github.com/SaraGhazanfari/LipSim.

==> figs/figure2.tex <==
\begin{figure}[t]
    \begin{minipage}{.45\textwidth}
    \centering
    xxx
    % \setlength\tabcolsep{1.5pt}
    % \begin{tabular}{cccc}
    %     \smallimg{figs/pgd_adv_images/original/7.pdf} &
    %     \smallimg{figs/pgd_adv_images/adv/7.pdf} &
    %     \smallimg{figs/pgd_adv_images/original/22.pdf} &
    %     \smallimg{figs/pgd_adv_images/adv/22.pdf} \\
    %     \multicolumn{2}{c}{$1.05$} & \multicolumn{2}{c}{$0.83$} \\
    %     \smallimg{figs/pgd_adv_images/original/23.pdf} &
    %     \smallimg{figs/pgd_adv_images/adv/23.pdf} &
    %     \smallimg{figs/pgd_adv_images/original/26.pdf} &
    %     \smallimg{figs/pgd_adv_images/adv/26.pdf} \\
    %     \multicolumn{2}{c}{$0.87$} & \multicolumn{2}{c}{$1.06$} \\
    %     \smallimg{figs/pgd_adv_images/original/65.pdf} &
    %     \smallimg{figs/pgd_adv_images/adv/65.pdf} &
    %     \smallimg{figs/pgd_adv_images/original/93.pdf} &
    %     \smallimg{figs/pgd_adv_images/adv/93.pdf} \\ 
    %     \multicolumn{2}{c}{$0.88$} & \multicolumn{2}{c}{$1.08$} \\
    % \end{tabular}
    % \caption{Original (left) and adversary images (right) generated using PGD-$\ell_{2}$ attack. The DreamSim distance between pairs of images is reported below them. \textcolor{red}{remove and place hist Fig 2 here}} 
    % \label{fig:pgd_adv_images}
    % \smallimg{figs/pgd_adv_images/original/7.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/adv/7.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/original/22.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/adv/22.pdf}\hfill\\
    % \begin{minipage}{3cm}
    % \centering
    % 1.05
    % \end{minipage}\hfill
    % \begin{minipage}{3cm}
    % \centering
    % 0.83
    % \end{minipage}\hfill
    % \smallimg{figs/pgd_adv_images/original/23.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/adv/23.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/original/26.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/adv/26.pdf}\hfill\\
    % \begin{minipage}{3cm}
    % \centering
    % 0.87
    % \end{minipage}
    % \begin{minipage}{3cm}
    % \centering
    % 1.06
    % \end{minipage}
    % \hfill
    % % \smallimg{figs/pgd_adv_images/original/32.pdf}
    % % \smallimg{figs/pgd_adv_images/adv/32.pdf}
    % % \smallimg{figs/pgd_adv_images/original/53.pdf}
    % % \smallimg{figs/pgd_adv_images/adv/53.pdf}\\
    % % \begin{minipage}{3cm}
    % % \centering
    % % 0.81
    % % \end{minipage}
    % % \begin{minipage}{3cm}
    % % \centering
    % % 0.96
    % % \end{minipage}
    % % \hfill
    % \smallimg{figs/pgd_adv_images/original/65.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/adv/65.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/original/93.pdf}\hfill
    % \smallimg{figs/pgd_adv_images/adv/93.pdf}\hfill\\    
    % \begin{minipage}{3cm}
    % \centering
    % 0.88
    % \end{minipage}\hfill
    % \begin{minipage}{3cm}
    % \centering
    % 1.08
    % \end{minipage}
    % \hfill
\end{minipage}%
\hfill
\begin{minipage}{.52\textwidth}
\flushleft
\includegraphics[scale=0.34,trim={2cm 1cm 2cm 1cm},clip]{figs/hist.pdf}
\caption{Histogram of $d(f(x), f(x+\delta))$. For feature extractor $f$ DreamSim Ensemble, Dino, and OpenClip are employed. Dino is showing more robustness than OpenClip and DreamSim Ensemble.}
\label{fig:histogram}
\end{minipage}
\end{figure}

==> figs/proposition1_figs.tex <==
\begin{figure}
    \centering
    \setlength\tabcolsep{1.5pt}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccccccc}
    \multicolumn{1}{r}{\multirow{1}{*}[0.3cm]{\Ronesymb}} &
    \img{figs/pro1_adv_imgs/original/3.pdf} &
    \img{figs/pro1_adv_imgs/original/5.pdf} &
    \img{figs/pro1_adv_imgs/original/36.pdf} &
    \img{figs/pro1_adv_imgs/original/40.pdf} &
    \img{figs/pro1_adv_imgs/original/57.pdf} &
    \img{figs/pro1_adv_imgs/original/61.pdf} &
    \img{figs/pro1_adv_imgs/original/80.pdf} &
    \img{figs/pro1_adv_imgs/original/139.pdf} &
    \img{figs/pro1_adv_imgs/original/196.pdf} \\
    \multicolumn{1}{r}{\multirow{1}{*}[0.3cm]{\Rtwosymb}} &
    \img{figs/pro1_adv_imgs/L2/3.pdf} &
    \img{figs/pro1_adv_imgs/L2/5.pdf} &
    \img{figs/pro1_adv_imgs/L2/36.pdf} &
    \img{figs/pro1_adv_imgs/L2/40.pdf} &
    \img{figs/pro1_adv_imgs/L2/57.pdf} &
    \img{figs/pro1_adv_imgs/L2/61.pdf} &
    \img{figs/pro1_adv_imgs/L2/80.pdf} &
    \img{figs/pro1_adv_imgs/L2/139.pdf} &
    \img{figs/pro1_adv_imgs/L2/196.pdf} \\
    \multicolumn{1}{c}{{\tiny $d(\text{\Ronesymb}, \text{\Rtwosymb})$}} 
    & {\tiny 0.65} & {\tiny 0.67} & {\tiny 0.64} & {\tiny 0.74} & {\tiny 0.65} & {\tiny 0.63} & {\tiny 0.65} & {\tiny 0.64} & {\tiny 0.55} \\
    \multicolumn{1}{r}{\multirow{1}{*}[0.3cm]{\Rthreesymb}} &
    \img{figs/pro1_adv_imgs/original/209.pdf} &
    \img{figs/pro1_adv_imgs/original/224.pdf} &
    \img{figs/pro1_adv_imgs/original/528.pdf} &
    \img{figs/pro1_adv_imgs/original/240.pdf} &
    \img{figs/pro1_adv_imgs/original/243.pdf} &
    \img{figs/pro1_adv_imgs/original/578.pdf} &
    \img{figs/pro1_adv_imgs/original/258.pdf} &
    \img{figs/pro1_adv_imgs/original/588.pdf} &
    \img{figs/pro1_adv_imgs/original/590.pdf} \\
    \multicolumn{1}{r}{\multirow{1}{*}[0.3cm]{\Rfoursymb}} &
    \img{figs/pro1_adv_imgs/L2/209.pdf} &
    \img{figs/pro1_adv_imgs/L2/224.pdf} &
    \img{figs/pro1_adv_imgs/L2/528.pdf} &
    \img{figs/pro1_adv_imgs/L2/240.pdf} &
    \img{figs/pro1_adv_imgs/L2/243.pdf} &
    \img{figs/pro1_adv_imgs/L2/578.pdf} &
    \img{figs/pro1_adv_imgs/L2/258.pdf} &
    \img{figs/pro1_adv_imgs/L2/588.pdf} &
    \img{figs/pro1_adv_imgs/L2/590.pdf} \\
    \multicolumn{1}{c}{{\tiny $d(\text{\Rthreesymb}, \text{\Rfoursymb})$}} 
    & {\tiny 0.62} & {\tiny 0.62} & {\tiny 0.64} & {\tiny 0.62} & {\tiny 0.65} & {\tiny 0.85} & {\tiny 0.6} & {\tiny 0.8} & {\tiny 0.71} \\
    \end{tabular}}
  \caption{\textbf{DreamSim violation of general robustness (Proposition~\ref{prop:prop_distance})} Instances of original and adversarial reference images, generated with $\ell_2$-AA ($\epsilon=0.5$). The DreamSim distance between them (\ie, $d(\text{\Ronesymb}, \text{\Rtwosymb})$ and $d(\text{\Rthreesymb}, \text{\Rfoursymb})$) is reported below, which is bigger than the perturbation budget and demonstrates the consequences of employing a perceptual metric that doesn't hold the general robustness. } % The adversary images are generated using AA-$\ell_2$ ($\epsilon=3.0$)}
  \label{fig:proposition1_fig}
\end{figure}
% \multicolumn{1}{c}{{\tiny $d(\text{\Ronesymb}, \text{\Rtwosymb})$}} 
% & {\tiny 0.43} & {\tiny 0.78} & {\tiny 0.66} & {\tiny 0.56} & {\tiny 0.81} & {\tiny 0.69} & {\tiny 0.78} & {\tiny 0.59} & {\tiny 0.86} \\[-0.1cm]
% % \midrule


==> tables/attack_acc.tex <==
\begin{table}[t]
\caption {Alignment on NIGHT dataset for original and perturbed images using AutoAttack. In this experiment, the perturbation is only applied on the reference images. While DreamSim employs an ensemble of three ViT-based model as the feature extractors, LipSim Backbone cosists of a 1-Lipschitz network (constituted of CNN and Linear layers) and is trained from scratch using the knowledge distillation approach.}
  \centering
    \begin{tabular}{lcrrrrr}
  \toprule
  \multirow{2}{*}{\textbf{Metric}}  & \multirow{2}{*}{\makecell{\textbf{Natural} \\ \textbf{Score}}} & \multicolumn{4}{c}{\textbf{$\ell_{2}$-AA}} \\
  \cmidrule{3-6}
   & & 0.5 & 1.0 & 2.0 & 3.0 \\
  \midrule
  \textbf{CLIP}    & 93.91 &  29.93 & 8.44 & 1.20 & 0.27 \\
  \textbf{OpenCLIP} & 95.45 &  72.31 & 42.32 & 11.84 & 3.28\\
  \textbf{DINO}    & 94.52 &  \textbf{81.91} & 59.04 & 19.29 & 6.35 \\
  \textbf{DreamSim Ensemble}  & 96.16 & 46.27 &  16.66 & 0.93 & 0.93 \\
  \midrule
  \textbf{LipSim (ours)}  & 85.09  & 81.58 & \textbf{76.92} & \textbf{65.62} & \textbf{53.07} \\
  \bottomrule
  \end{tabular}
  \label{tab:adv_results}
\end{table}

==> tables/attack_acc_full.tex <==
\begin{table}[t]
\caption {}
  \centering
    \begin{tabular}{ccccccc}
  \cmidrule[1pt]{2-7}
  & Metric  & \multirow{2}{*}{\makecell{\textbf{Natural} \\ \textbf{Score}}} & \multicolumn{4}{c}{\textbf{$\ell_{2}$-AA}}\\
  \cmidrule{4-7}
   & & & 0.5 & 1.0 & 2.0 & 3.0 \\
  \cmidrule[1pt]{2-7}
  & \textbf{DINO}    & 94.52 &  81.91 & 59.04 & 19.29 & 6.35 \\
  & \textbf{CLIP}    & 93.91 &  29.93 & 8.44 & 1.20 & 0.27\\
  & \textbf{OpenCLIP} & 95.45 &  72.31 & 42.32 & 11.84 & 3.28\\
  & \textbf{LPIPS}  & 70.7 & xxx &  xxx & xxx & xxx \\
  & \textbf{DreamSim}  & 96.16 & 46.27 &  16.66 & 0.93 & 0.93 \\
  & \textbf{LipSim}  & 85.09  & 81.58 & 76.92 & 65.62 & 53.07\\
  
   \cmidrule[1pt]{2-7}
  \end{tabular}
  \label{tab:full_adv_results}
\end{table}

==> tables/certified_acc_full.tex <==
\begin{table}[t]
\caption {Certified Accuracy}
  \centering
    \begin{tabular}{cccccccc}
  \cmidrule[1pt]{2-8}
  & \multirow{2}{*}{\makecell{Teacher \\ model}} & version & Margin & \multirow{2}{*}{\makecell{\textbf{Natural} \\ \textbf{Score}}} & \multicolumn{3}{c}{\textbf{Certified Score}}\\
  \cmidrule{6-8}
  &&&&&$\frac{36}{255}$ & $\frac{72}{255}$ & $\frac{108}{255}$\\
  \cmidrule[1pt]{2-8} 
  & \multirow{3}{*}{\textbf{DINO}}   & pretrained  & - & 86.90 & 53.67 & 17.32 & 2.25 \\
  \cmidrule{4-8}
      % &   & \multirow{3}{*}{finetuned}  & 0.1 & 84.10 & 61.02 & 28.5 & 7.46 \\
      
    &   & \multirow{2}{*}{finetuned}  & 0.2 & 88.87 & 63.54 & 29.88 & 7.29 \\
    % &   &   & 0.3 & 88.27 & 63.76 & 33.28 & 9.37\\
    % &   &   & 0.4 & 87.66 & 67.16 & 37.23 & 11.51\\
    &   &   & 0.5 & 86.18 & 66.17 & 41.01 & 17.32\\
    \cmidrule{3-8}
  & \multirow{3}{*}{\textbf{OpenCLIP}} & pretrained & - & 79.06 & 41.17 & 10.58 & 0.88 \\
  \cmidrule{4-8}
  % &   &   & 0.1 & 83.83 & 59.59 & 30.76 & 10.03\\
    &   & \multirow{2}{*}{finetuned}  & 0.2 & 82.51 & 61.35 & 34.32 & 12.50\\
    % &   &   & 0.3 & 84.54 & 63.27 & 36.68 & 14.09\\
    % &   &   & 0.4 & 83.44 & 62.23 & 38.60 & 16.83\\
    &   &   & 0.5 & 81.90 & 62.72 & 39.75 & 19.57\\
\cmidrule{3-8}
& \multirow{3}{*}{\textbf{Ensemble}} & pretrained & - & 86.62 & 52.14 &  16.56 & 1.81\\
\cmidrule{4-8}
% &   & \multirow{3}{*}{finetuned}  & 0.1 &  84.32 & 60.08 & 29.39 & 7.67\\
    &   & \multirow{2}{*}{finetuned}  & 0.2 &  88.60 & 64.47 & 31.85 & 9.43\\
    % &   &   & 0.3 &  87.34 & 66.44 & 34.43 & 11.02 \\
    % &   &   & 0.4 & 87.39 & 66.89 & 37.94 & 15.37\\
    &   &   & 0.5 & 85.09 & 67.32 & 43.26 & 19.02\\
   \cmidrule[1pt]{2-8}
  \end{tabular}
  \label{tab:adv_results}
\end{table}

